LayoutVLM: Differentiable Optimization of 3D Layout via Vision-Language Models

Spatial reasoning is a fundamental aspect of human cognition, enabling intuitive understanding and manipulation of objects in three-dimensional space. While foundation models demonstrate remarkable performance on some benchmarks, they still struggle with 3D reasoning tasks like arranging objects in space according to open-ended language instructions, particularly in dense and physically constrained environments. We introduce LayoutVLM, a framework and scene layout representation that exploits the semantic knowledge of Vision-Language Models (VLMs) and supports differentiable optimization to ensure physical plausibility. LayoutVLM employs VLMs to generate two mutually reinforcing representations from visually marked images, and a self-consistent decoding process to improve VLMs spatial planning. Our experiments show that LayoutVLM addresses the limitations of existing LLM and constraint-based approaches, producing physically plausible 3D layouts better aligned with the semantic intent of input language instructions. We also demonstrate that fine-tuning VLMs with the proposed scene layout representation extracted from existing scene datasets can improve their reasoning performance.

==> figure-text/pull.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figure/overview.png}
    \caption{\textbf{figure to be updated.}}
    \label{fig:pull}
\end{figure*}

==> table-text/grammar.tex <==
% \begin{table*}[t]
% %\centering
% \small
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lll}
% \toprule
% \multicolumn{3}{l}{\textbf{Data Types}} \\ \midrule
% \textbf{Name} & \textbf{Type} & \textbf{Description} \\ \midrule
% \texttt{Wall} & \texttt{BaseModel} & Wall with attributes \texttt{corner1}, \texttt{corner2}, and optional \texttt{instance\_id}. \\ 
% \texttt{AssetInstance} & \texttt{BaseModel} & 3D asset instance with attributes \texttt{optimize}, \texttt{position}, \texttt{rotation}, and optional \texttt{instance\_id}. \\
% \texttt{Assets} & \texttt{BaseModel} & Collection of 3D asset instances with \texttt{description}, \texttt{placements}, and optional \texttt{size}. \\ 
% \texttt{Constraint} & \texttt{Class} & Defines constraints with \texttt{constraint\_name} and optional \texttt{params}. \\ 
% \texttt{ConstraintSolver} & \texttt{Class} & Solver to manage and enforce spatial constraints among assets and walls. \\ 
% %\texttt{get\_instance\_id} & \texttt{Function} & Retrieves unique identifier of an asset or wall instance. \\ 
% \end{tabular}
% }

% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lll}
% \toprule
% \multicolumn{3}{l}{\textbf{Grammar}} \\
% \midrule
% \textbf{Syntax} & \textbf{Definition} & \textbf{Description} \\ 
% \midrule
% \texttt{align\_with} & \texttt{(asset1, asset2, angle)} & Aligns two assets with a specified angle. \\ 
% \texttt{point\_towards} & \texttt{(asset1, asset2, angle)} & Orients one asset to face another at a specified angle. \\
% \texttt{against\_wall} & \texttt{(asset, wall)} & Places an asset adjacent to a specified wall. \\
% \texttt{distance\_constraint} & \texttt{(asset1, asset2, min\_distance, max\_distance)} & Enforces a distance constraint between two assets. \\ 
% \texttt{on\_top\_of} & \texttt{(asset1, asset2)} & Positions one asset on top of another. \\ 
% \end{tabular}
% }

% \resizebox{\linewidth}{!}{%
% \begin{tabular}{ll}
% \toprule
% \multicolumn{2}{l}{\textbf{Macros}} \\ \midrule
% \textbf{Macro} & \textbf{Description} \\ \midrule
% \texttt{get\_instance\_id} & Returns the unique identifier of an asset or wall instance based on type and instance details. \\ 
% \bottomrule
% \end{tabular}
% }
% % \resizebox{\linewidth}{!}{%
% % \begin{tabular}{ll}
% % \toprule
% % \multicolumn{2}{l}{\textbf{Special Forms}} \\ \midrule
% % \bottomrule
% % \end{tabular}
% % }
% \caption{The Domain-Specific Language. This table defines the data types, grammar, macros, and special forms used in the DSL to manage asset placement and spatial constraints.}
% \label{table:dsl_components}

% \end{table*}

\begin{table*}[t]
\small % This sets the font size consistently for all tables


\begin{tabularx}{\linewidth}{llX}
\toprule
\multicolumn{3}{l}{\textbf{Data Types}} \\
\midrule
\textbf{Name} & \textbf{Type} & \textbf{Description} \\
\midrule
\texttt{Wall} & \texttt{BaseModel} & Wall with attributes \texttt{corner1}, \texttt{corner2}, and optional \texttt{instance\_id}. \\
\texttt{AssetInstance} & \texttt{BaseModel} & 3D asset instance with attributes \texttt{optimize}, \texttt{position}, \texttt{rotation}, and optional \texttt{instance\_id}. \\
\texttt{Assets} & \texttt{BaseModel} & Collection of 3D asset instances with \texttt{description}, \texttt{placements}, and optional \texttt{size}. \\
\texttt{Constraint} & \texttt{Class} & Defines constraints with \texttt{constraint\_name} and optional \texttt{params}. \\
\texttt{ConstraintSolver} & \texttt{Class} & Solver to manage and enforce spatial constraints among assets and walls. \\
%\bottomrule
\end{tabularx}

\begin{tabularx}{\linewidth}{llX}
\toprule
\multicolumn{3}{l}{\textbf{Grammar}} \\
\midrule
\textbf{Syntax} & \textbf{Definition} & \textbf{Description} \\
\midrule
\texttt{align\_with} & \texttt{(asset1, asset2, angle)} & Aligns two assets with a specified angle. \\
\texttt{point\_towards} & \texttt{(asset1, asset2, angle)} & Orients one asset to face another at a specified angle. \\
\texttt{against\_wall} & \texttt{(asset, wall)} & Places an asset adjacent to a specified wall. \\
\texttt{distance\_constraint} & \texttt{(asset1, asset2, min\_distance, max\_distance)} & Enforces a distance constraint between two assets. \\
\texttt{on\_top\_of} & \texttt{(asset1, asset2)} & Positions one asset on top of another. \\
%\bottomrule
\end{tabularx}

\begin{tabularx}{\linewidth}{lX}
\toprule
\multicolumn{2}{l}{\textbf{Macros}} \\
\midrule
\textbf{Macro} & \textbf{Description} \\
\midrule
\texttt{get\_instance\_id} & Returns the unique identifier of an asset or wall instance based on type and instance details. \\
\bottomrule
\end{tabularx}

\caption{The Domain-Specific Language. This table defines the data types, grammar, macros, and special forms used in the DSL to manage asset placement and spatial constraints.}
\label{table:dsl_components}
\end{table*}

==> table-text/rebuttal_ablation.tex <==
\begin{table}[t]
    \centering%\small
    % \tiny
    \setlength\tabcolsep{4pt}
    \setlength\extrarowheight{1pt}
    \begin{adjustbox}{width=\linewidth}
    % \setlength{\tabcolsep}{1pt}
    % \resizebox{\columnwidth}{!}{%
    %\scriptsize
    \begin{tabular}{lccccc}
    \hline
     & \multicolumn{2}{c}{Physics} & \multicolumn{2}{c}{Semantics} & \multicolumn{1}{c}{Overall Score} \\
    \cline{2-3} \cline{4-5}  \cline{6-6}
    & CF & IB & Pos. & Rot. & PSA\\
    \hline
    \method & \textbf{81.8 $\pm$ 2.5} &  \textbf{94.9 $\pm$ 2.2} &  77.5 $\pm$   0.9 &  \textbf{73.1 $\pm$ 1.1} &  \textbf{58.8 $\pm$ 3.4}\\
    \midrule
   w/o Visual Asset Mark & 79.8 $\pm$   0.6 &  87.9 $\pm$   3.9 &  \textbf{77.7 $\pm$   0.6} &  72.2 $\pm$   0.8 &  52.2 $\pm$   5.0   \\
    w/o Visual Coordinate  &  77.2 $\pm$   2.0 &  88.9 $\pm$   1.7 &  74.3 $\pm$   1.0 &  68.9 $\pm$   1.3 &  46.0 $\pm$   2.7 \\
    w/o Any Visual Mark &  74.2 $\pm$   6.4 &  84.9 $\pm$   3.1 &  74.5 $\pm$   0.8 &  69.2 $\pm$   0.3 &  43.0 $\pm$   2.2 \\
    \midrule
    w/o Numerical Init. & 74.7 $\pm$   4.0 &  86.6 $\pm$   2.6 &  69.5 $\pm$   0.1 &  65.4 $\pm$   1.4 &  41.0 $\pm$   1.7 \\
    w/o (Spatial) Const.  & 75.8 $\pm$   2.5 &  14.1 $\pm$   3.0 &  70.4 $\pm$   1.3 &  67.3 $\pm$   0.9 &   6.7 $\pm$   1.6 \\
    \hline
    \end{tabular}
    %}
    \end{adjustbox}
    \vspace{-10pt}
    \caption{Additional ablation studies on Visual Mark and the proposed Scene Layout Representation, averaged over the entire dataset (i.e., 11 room types $\times$ 3 rooms $\times$ 3 seeds $\times$ 3 runs).}
    %\vspace{-1mm}
    \label{tab:ablation_more}
\end{table}

